CodeSense: a Real-World Benchmark and Dataset for Code Semantic Reasoning

Understanding and reasoning about code semantics is essential for enhancing code LLMs' abilities to solve real-world software engineering (SE) tasks. Although several code reasoning benchmarks exist, most rely on synthetic datasets or educational coding problems and focus on coarse-grained reasoning tasks such as input/output prediction, limiting their effectiveness in evaluating LLMs in practical SE contexts. To bridge this gap, we propose CodeSense, the first benchmark that makes available a spectrum of fine-grained code reasoning tasks concerned with the software engineering of real-world code. We collected Python, C and Java software projects from real-world repositories. We executed tests from these repositories, collected their execution traces, and constructed a ground truth dataset for fine-grained semantic reasoning tasks. We then performed comprehensive evaluations on state-of-the-art LLMs. Our results show a clear performance gap for the models to handle fine-grained reasoning tasks. Although prompting techniques such as chain-of-thought and in-context learning helped, the lack of code semantics in LLMs fundamentally limits models' capabilities of code reasoning. Besides dataset, benchmark and evaluation, our work produced an execution tracing framework and tool set that make it easy to collect ground truth for fine-grained SE reasoning tasks, offering a strong basis for future benchmark construction and model post training. Our code and data are located at https://codesense-bench.github.io/.

==> Bakeup/abst.tex <==
\begin{abstract}

\gail{ The ML community had already been hearing about machine learning models for "code understanding" for several years before GPT.  MANY papers claimed that previous work was based only on programming language syntax, but the paper's new idea is different because it leverages semantics in a way that enables a big breakthrough towards automating a wide range of software engineering tasks. So what is new and different about this paper that was not already addressed by the dozens if not hundreds of other ML4Code or ML4SE papers published in the past eight years? Note we have to make a case that this new paper improves in some way (is the first to do xxx) than our own previous papers like SemCoder and TRACED, plus any papers by Wei that I may not know about - referring to all these as if work by unrelated people because of anonymity rules. }

Motivation: ML community may not know the meaning of input/output prediction 
we need to give a whole story in motivation from application why this is important 

evaluate whether or not the model learns the semantics of code. the accuracy of SE tasks (debugging, vulnerability detection, generate larger code) relies on understanding the precise semantics than just code summarization
- Probe: the model understands the code, they can do more things that program analysis can do

Natural language explain what does this statement do? (operational semantics) - difficult to evaluate, no ground truth, no fine-grained statement level evaluation of code semantics)


Contributions: enable automatic evaluation of fine-grained code semantics using traced benchmarks and dataset 
\begin{enumerate}
\item dataset (real world code of three programming languages, an their traces) and tracing tools 
\item benchmark (novelty: tasks)
\begin{itemize}
\item Precise concrete semantic probing: Stepwise intermediate value prediction: to understand the impact of sizes and types of statements on models 
\begin{itemize}
\item given an input of a statement, predict the output of the statement
\item probe different types of statements: arithmetic, branches, loops, calls (values after API, system calls - networks, user defined functions), Language specific Java: virtual target prediction, which target 
\item increases the sizes of statements: from one, two ... to the entire functions 
\item special sizes and types of statements
- Branch outcome for given input 
- Loop count (range)
- Loop values (in loop, after loop)
\end{itemize}

\item Approximate concrete semantic probing: quantized values 

\item Abstract semantic probing: reason for all program behaviors
Query driven with application in mind
- dependency: 
-- is this value tainted 
-- Function A dependent on function B? (big context check)
-- Output dependent on the input?
-- Intermediate value dependent on the input
-- Values after API dependent on the input of API 

- Is this pointer can be null?
\end{itemize}

\item thorough evaluation:
raw, fine-tuning, RAG, prompt engineering 
\end{enumerate}


LLM cannot handle SE tasks very well. Vulnerability detection. These tasks are complicated and require low level elements





{construct benchmark based on tasks}
Easy, medium, difficult: three categories 
Related work:
https://dl.acm.org/doi/pdf/10.1145/3649828
Bigcodebench
Livecodebench


define code reasoning tasks
abstract program properties in the low level elements that general for all programs

dependencies
branch prediction (given one branch to predict another)
loops (iterations, values after loops)
aliaing
NULL pointers 
Dataflow properties


\begin{itemize}
\item dataset (multilingual, source code, traces, abstract traces (configurable) - traced paper, framework to generate more traces, readme (how to run), appendix -- framework and dataset outline)
Numbers of programs: 
Java: 40 projects
C/C++: 400 programs
Python: 

\item benchmark - code understanding (real-world, fine-grained information)
Motivation: semantics, debugging, repair
Tasks: 
- input/output, intermediate values (random sample based on the variable types), branches 
- build/execution environment

Metrics: F1

Numbers of programs: 20 
Types: branch complexity (variable types considered)
- simple 
- medium
- complex ones 

\item research questions 
\begin{itemize}
\item HumanEval trace helped CruxEval: reduce counterfeit (code generation)
\item realworld trace (how many traces?) (simple, python, needed) helped CruxEval more?
\item HumanEval traces helped our benchmark (simple, python)?
\item realworld (abstract traces) helped our benchmark?
\end{itemize}
\end{itemize}

Yes: improvement - motivation of our work
No: explanations, why not work and what to improve

CruxEval paper

We propose 
(1) a new multilingual real-world project execution trace dataset for training models with execution traces
(2) an evaluation benchmark dataset
(3) a framework to generate the dataset
\end{abstract}


==> Bakeup/checklist-back.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}



==> Bakeup/intro-Ray.tex <==
\section{Introduction}

Semantic code reasoning—the capacity to understand and predict the behavior of programs—is a core requirement for advanced code generation systems. It underpins a wide range of complex software engineering tasks, including test input generation, vulnerability detection, fault localization, program repair, refactoring, and functional verification. Unlike syntactic pattern matching, which may rely on token-level similarity or statistical regularities, semantic reasoning entails a deep, execution-oriented understanding of how programs operate. Although code semantics can be expressed in many ways, in practice, developers engage in semantic reasoning through tasks like predicting a function’s input-output behavior, tracing variable values, analyzing control flow paths, identifying loop invariants, etc. This form of reasoning aligns with formal definitions from programming language theory—particularly operational semantics, which models step-by-step execution, and axiomatic semantics, which uses logical assertions to describe program properties. Such reasoning tasks also reflect the real-world demands placed on developers and provide a natural grounding for \wei{LLMs' code generation and reasoning}.

% Recent years have seen a rise in coding task related benchmarks. However, a majority of them are focused on code generation tasks–HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased} using synthetic data or isolated competitive programming context. Thus, these benchmarks fail to reflect the complexity of real-world software engineering. Second,  benchmarks using real-world code, like  SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}, tend to focus on specific end-user tasks (e.g., patch generation), making it difficult to determine whether models possess generalizable semantic understanding. Finally, reasoning-focused benchmarks such as CruxEval~\cite{gu2024cruxevalbenchmarkcodereasoning} evaluate only coarse-grained tasks like function-level I/O prediction over short, synthetically generated code performing random string operations, while neglecting fine-grained semantic reasoning needed for understanding internal program behavior, data flow, or control structures in real-world complex software. 


% --
% Semantic code reasoning—the capacity to understand and predict the behavior of programs—is a fundamental requirement for advanced code generation systems. It supports a broad range of complex software engineering tasks, including debugging, bug localization and repair, refactoring, and functional verification. In contrast to syntactic pattern matching, which often relies on token-level similarity or statistical correlations, semantic reasoning demands a deep, execution-aware understanding of program behavior.

% Although code semantics can be formalized in multiple ways, such as operational, denotational, or axiomatic semantics, developers in practice engage in semantic reasoning through tasks like predicting a function’s input-output behavior, tracing variable values, analyzing control flow, and identifying loop invariants. These forms of reasoning not only align with foundational definitions from programming language theory—especially operational semantics, which models execution as state transitions, and axiomatic semantics, which characterizes program correctness through logical assertions—but also reflect the day-to-day cognitive demands placed on developers. As such, they provide a meaningful foundation for evaluating the semantic competence of code generation models.


Recent years have witnessed the emergence of numerous benchmarks for evaluating coding-related tasks. However, the majority of these efforts have focused on code generation using synthetic or narrowly scoped data—for example, HumanEval+~\cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark~\cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench~\cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, and CodeBenchGen~\cite{xie2024codebenchgencreatingscalableexecutionbased}—often grounded in isolated competitive programming problems. Consequently, they fail to capture the complexity and structure of real-world software development. Other benchmarks that incorporate real-world code, such as SWE-Bench~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}, tend to evaluate task-specific performance (e.g., patch generation for GitHub issues), making it difficult to assess whether models exhibit generalizable semantic understanding. Finally, reasoning-focused benchmarks such as CruxEval~\cite{gu2024cruxevalbenchmarkcodereasoning}, primarily targets function-level input/output prediction over short, synthetic code fragments involving random string operations. Such settings neglect the fine-grained semantic reasoning required to understand internal program behavior, data dependencies, and control structures in real-world complex software systems.


% Recent years have witnessed the emergence of numerous benchmarks for evaluating coding-related tasks. However, the majority of these efforts have focused on code generation using synthetic or narrowly scoped data—for example, HumanEval+~\cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark~\cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench~\cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, and CodeBenchGen~\cite{xie2024codebenchgencreatingscalableexecutionbased}—often grounded in isolated competitive programming problems. Consequently, they fail to capture the complexity and structure of real-world software development.

% Other benchmarks that incorporate real-world code, such as SWE-Bench~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}, tend to evaluate task-specific performance (e.g., patch generation for GitHub issues), making it difficult to assess whether models exhibit generalizable semantic understanding.

% Finally, reasoning-focused benchmarks such as CruxEval~\cite{gu2024cruxevalbenchmarkcodereasoning} remain limited in scope. CruxEval, for instance, primarily targets function-level input/output prediction over short, synthetic code fragments involving random string operations. Such settings neglect the fine-grained semantic reasoning required to understand internal program behavior, data dependencies, and control structures in large-scale, real-world software systems.


% Currently, we see gaps in code benchmark design: (1) \textit{lacking real-world code sources}:  benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}~\ray{is it also competitive coding benchmark?}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}   used synthetic data or stand-alone competitive coding problems, which do not reflect how developers develop large scale software in real world; %.  and the evaluation is not centered on real-world software projects; 
% (2) \textit{focusing on coarse-grained simple reasoning tasks}: benchmarks like 
% CruxEval ~\cite{gu2024cruxevalbenchmarkcodereasoning} focused on simple tasks such as input/output prediction at a function level (where functions are simple few lines code using string utility);  however, there are many other code reasoning tasks, many of which require to reason about fine-grained code semantics like the values of statements and properties within a function (3) \textit{evaluating a limited set of end-user tasks for real-world code}:  SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}  are the benchmarks we found that use real-world code (to the best of our knowledge). However, these benchmarks focus on task-specific evaluation rather than directly assessing whether a model understands code semantics. Using such benchmarks, we may learn whether the model performs well for a particular end-user task such as generating patches to resolve a GitHub issue; but it is unclear when the models improve performance on such tasks, whether they can also perform better on many other SE tasks.



% Currently, we see gaps in code benchmark design: (1) \textit{lacking real-world code sources}:  benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}~\ray{is it also competitive coding benchmark?}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}   used synthetic data or stand-alone competitive coding problems, which do not reflect how developers develop large scale software in real world; %.  and the evaluation is not centered on real-world software projects; 
% (2) \textit{focusing on coarse-grained simple reasoning tasks}: benchmarks like 
% CruxEval ~\cite{gu2024cruxevalbenchmarkcodereasoning} focused on simple tasks such as input/output prediction at a function level (where functions are simple few lines code using string utility);  however, there are many other code reasoning tasks, many of which require to reason about fine-grained code semantics like the values of statements and properties within a function (3) \textit{evaluating a limited set of end-user tasks for real-world code}:  SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}  are the benchmarks we found that use real-world code (to the best of our knowledge). However, these benchmarks focus on task-specific evaluation rather than directly assessing whether a model understands code semantics. Using such benchmarks, we may learn whether the model performs well for a particular end-user task such as generating patches to resolve a GitHub issue; but it is unclear when the models improve performance on such tasks, whether they can also perform better on many other SE tasks.

%----when models perform poorly, it is hard to understand why and which step that prevents the models from performing better.

%To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.
To this end, we propose \bench, a benchmark for fine-grained code semantic reasoning, constructed from real-world GitHub projects in Python, C, and Java. \bench~introduces a spectrum of reasoning tasks at statement, code-block, and function levels, targeting essential semantic properties frequently needed across software engineering (SE) applications. To enable supervised evaluation, we develop a framework that automatically extracts ground-truth annotations for these tasks using static and dynamic program analysis. For example, predicting loop iteration counts is critical for I/O reasoning, performance analysis, and detecting infinite loops (e.g., denial-of-service vulnerabilities). Other tasks include branch condition prediction and memory error localization, which require models to reason across arithmetic operations, control flow, and API semantics. As illustrated in Figures~\ref{fig:test} and~\ref{fig:vul}, such semantic reasoning is foundational for tasks like input or test-case generation, fault localization, and automated program repair. Prior work~\cite{ding2023tracedexecutionawarepretrainingsource,ding2024semcodertrainingcodelanguage} has shown that incorporating semantic signals during training improves model performance on diverse SE tasks,  including code generation, branch prediction, code clone detection, program repair and vulnerability detection, motivating our design of \bench as a comprehensive semantic reasoning benchmark.



%We propose \bench: (1) it is constructed from real-world GitHub software projects of Python, C and Java, (2) it introduced a spectrum of fine-grained {\it code semantic reasoning tasks} that are essential for a wide range of SE tasks. Using domain knowledge, we identified important, frequently needed code properties across multiple levels of code granularity, statement-level, block-level and function-level. We built a framework and tool chain that can generate ground truth for these fine-grained code reasoning tasks. For example, it is important to reason about loop iterations for input/output prediction, for identifying software performance bottleneck, and for also detecting denial-of-service (infinite loops) attacks. Thus, one of our fine-grained semantic reasoning tasks is to predict the number of loop iterations given an input. As another example, in Figure~\ref{fig:test}, to generate an input to test the dangerous code at line~4, we need the model to understand the code semantics of arithmetic at line~2 and the conditional branch at line~3, so that it can construct a value to set the branch to be {\tt true}. Such statement level code semantic understanding is also important for SE applications like branch prediction and input/output prediction. Similarly, in Figure~\ref{fig:vul}, the models need to understand the semantics of calls {\tt malloc} and {\tt free} at lines~2 and 4, as well as the branch at line 3 o detect whether this code has a memory leak to localize the fault, and to repair it. In the prior literature Traced~\cite{ding2023tracedexecutionawarepretrainingsource} and SemCoder~\cite{ding2024semcodertrainingcodelanguage}, researchers have demonstrated that fine-tuning models with code semantics, the models can improve a variety of SE tasks, including code generation, branch prediction, code clone detection, program repair and vulnerability detection. 

\begin{figure}
% \begin{wrapfigure}{r}{0.65\textwidth}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
void foo(int input){
   int n = input * 23;
  if (n >= 1580){
     //dangerous code need to be tested 
  }
}
    \end{minted}
    \end{tcolorbox}
    \caption{Test input generation and execution reasoning: to generate a test input that can lead to the execution of dangerous code. The model needs to find an input that can make the condition $n\geq$ 1580 true. However, it is hard to generalize across examples, as each program can have different values, without knowing semantics, it is hard to find patterns. Understanding the semantics of operators '*' at line 2 an '$\geq$' at line 3 is needed to effectively generate test input that reaches dangerous code, e.g., n = 2000 \label{fig:test}}
    \end{subfigure}\quad%
    % 
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3,5,7,8},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
    void bar (int nbits) {
        FFTContext *s = malloc(sizeof (* s));
        if (s && nbits==100))
            free(& s);
         return s;
 }
    \end{minted}
    \end{tcolorbox}
    \caption{Vulnerability detection, fault localization and repair: this code has a memory leak vulnerability when the {\tt if} condition at line~3 is {\tt false}. To detect this vulnerability, it is best that the models know that calls of {\tt malloc} and {\tt free} are related to the vulnerability (semantics of the calls), and should be paired along the program paths along both branches of {\tt if} conditions (semantics of the branch statements). {\tt malloc} and {\tt free} can be located in various code context in different programs, it is hard to generalize the patterns from the code text only without code semantic reasoning.
    \label{fig:vul}}
    \end{subfigure}
    \definecolor{DiffGreen}{HTML}{368B00}
    \definecolor{DiffRed}{HTML}{A51901}
    \caption{Fine-grained code semantics are the keys for solving many SE tasks
    \label{fig:example}}
\end{figure}

%implementation
To construct \bench, we collected 544 Python, 100 C, 100 Java projects, we developed a comprehensive framework to build, execute and collect run-time execution values and traces of the real-world projects. 
%For Python, we executed test cases using the pytest module, and collected execution traces using PySnooper. For C, we used the projects curated in OSS-Fuzz, and the projects were built and fuzzed by OSS-fuzz's docker-based infrastructure. We employed GNU debugger(GDB) to collect run-time traces from C projects. For Java, We used the SF110 dataset, and EvoSuite to generate test cases. We developed the Java tracing framework using the Java Debugger. 

build, execute and collect run-time execution values and traces of the real-world projects.
Using the collected execution trace logs, we build analysis tools to extract the ground truth for our reasoning tasks, and applied filters (details in Section 3) and selected a total of 2125 Python,  876 C, and 875 Java unique functions in our benchmark.

%we constructed \bench, by extracting the function-level traces and curating benchmark datasets for different code understanding tasks.

%\wei{Roy please add some details regarding our benchmark construction and tools} 

%research question
Using our benchmark, we evaluated  SOTA LLMs and investigated six research questions regarding models code semantic reasoning capabilities. In the past, we see that models did not perform well on code reasoning tasks such as input/output prediction~\cite{gu2024cruxevalbenchmarkcodereasoning} and vulnerability detection~\cite{steenhoek2025errmachinevulnerabilitydetection}; to understand why models fail and identify places for improvement, we investigate:
\textbf{RQ1:} Which types of program statements are easier or harder for models to reason about? % in value prediction?  
\textbf{RQ2:} Does increasing code size make semantic reasoning more difficult?  
\textbf{RQ3:} How do models perform on code properties critical for SE tasks, such as pointer aliasing, loop iteration counts, and branch conditions?  
\textbf{RQ4:} How effective are different prompting strategies in improving semantic reasoning?  
\textbf{RQ5:} Do models perform better on some programming languages than others?  
\textbf{RQ6:} Can models reason approximately when exact values or semantics are hard to infer?


% {\bf RQ1}: {\it What types of program statements the model can understand well?  does the model feel any type particularly difficult?}  and {\bf RQ2:} {\it Does increasing the size of code increase the difficulty of code reasoning?}. We identified and evaluated frequently code reasoning tasks shared across many SE tasks, and investigated {\bf RQ3}: {\it How do models perform regarding code properties that are frequently needed for solving SE tasks such as pointer aliasing, loop iterations and values, and branch prediction?} We also studied {\bf RQ4}: {\it How do different prompt techniques help?} and {\bf RQ5}: {\it Any particular programming languages are easier for the models?}. We observed that models face challenges of predicting a precise program value/property, so  we investigated {\bf RQ6}: {\it Can models reason about an approximation of code semantics?}.
%%While the code reasoning capabilities of LLMs rapidly improve, to probe we are there yet, we studied {\bf RQ7}: {\it How does the best SOTA LLMs perform our fine-grained code reasoning tasks?}

%results
%\wei{Roy: can you add a summary of results}\\
Our results reveal that current LLMs, including state-of-the-art models like Claude 3.7, GPT-4o-mini, and Gemini 1.5, struggle with fine-grained code semantics. They often fail to reason accurately about even single statements from real-world code—particularly arithmetic expressions and API calls—and perform poorly on tasks involving loop values, iteration counts, and pointer aliasing. Basic chain-of-thought prompting offers limited benefit, and few-shot prompting yields only modest improvements unless carefully tailored to the query context. 
Interestingly, models demonstrate partial semantic understanding for frequently occurring patterns. For instance, when prompted with an explanation that assignments like {\tt p = q} indicate pointer aliasing, models correctly infer alias relationships even in zero-shot settings. Similarly, models reliably infer loop bounds in explicit cases such as {\tt for i in range(100):}. In-context learning is most effective when prompts define new semantic concepts or include highly relevant examples. Among the 14 models evaluated, Claude 3.7 consistently achieved the best performance. We also observe that Java and Python code are generally easier for models to reason about than C, and that input prediction (i.e., reverse semantic inference) remains among the most challenging tasks.


% Our results show that current LLMs lack sufficient knowledge of fine-grained code semantics and face challenges of reasoning for even one statement from real-world code, especially for arithmetic statements and API/calls. LLMs also generally reported low performance for reasoning about program properties such as loop values and iterations. The reasoning models and the state-of-the-art big models like Claude 3.7, GPT 4o-mini and Gemini-1.5, do not help much.  Simple COT prompting is not useful. Interestingly, the models do know some semantics for the frequently occurred code patterns, like when the code text contains an assignment "p=q", and our prompt explained that "two aliased pointers have the same memory addresses", the models are able to return {\tt p} and {\tt q} are aliased even in the zero-shot setting. Similarly, when our prompt asked the model to answer the number of loop iterations, the models often know they should report 100 if the code contains the loop {\tt for i in range(100):}. In context-learning prompting helped especially when we selected the in-context shots relevant to our queries, but the improvement is not significant. It is especially useful when we introduce a newly defined concept in the prompt, e.g., when we asked models to predict "abstract values" and we define what we mean by abstract values in the prompt. Among the 14 SOTA models we studied, we found that Claude 3.7 overall performed best in our fine-grained reasoning tasks.  We found that compared to C code, Java/Python are easier for models to predict output given input. Models have very little knowledge on "reverse" code semantcs, and input predictions becomes the most difficult tasks.

\mycomment{
We observed that reasoning is more difficult when the code size increase. We observed that across different programming languages, C is the most difficult for output prediction, python is the most for input prediction \wei{Roy, please double check this conclusions}. 
Good models: Claude, better models for all tasks  Granaite models
\wei{will  Models are able to link natural language in our prompt with code patterns, e.g., }
}

\noindent\textbf{Contributions.} This work introduces a realistic and comprehensive benchmark for evaluating LLMs' fine-grained code semantic reasoning in practical software engineering contexts. We advance the state of the art code reasoning benchmarks by:

\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item Defining a diverse set of fine-grained semantic reasoning tasks grounded in real-world software engineering needs.
\item Developing a scalable framework and toolchain to automatically generate program traces and semantic annotations, enabling continuous benchmark expansion while mitigating data leakage.
\item Constructing a benchmark dataset using real-world projects in Python, C, and Java.
\item Empirically analyzing six research questions across 14 state-of-the-art LLMs to assess their strengths and limitations in semantic reasoning.
\item Launching a public leaderboard to support reproducibility and accelerate progress on semantic reasoning for code.
\end{enumerate}


%exhibits varying capabilities across different semantic tasks. For RQ1, while the models show higher prediction accuracy for statements like Constant Assignment and branch statements, they struggle with tasks which involve function calls and arithmetic. We also observed that increasing block sizes resulted in a decrease in performance for the models (RQ2). 


%Our goal of designing \bench is to improve the state-of-the-art (SOTA) code benchmarks by (1) defining a spectrum of code semantic reasoning tasks that are important for a variety of SE tasks (2) delivering a framework and tool chain that can continuously produce new program traces and construct ground truth for code semantics for real-world software projects consisting of Python, C and Java, useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.


%his paper presents a comprehensive study and real-world multi-lingual benchmark, dataset and framework tools that can evaluate the future models. It's the first this paper is first that defines the code reasoning capabilities via a spectum of fine-grained code reasoning tasks that directly link to important SE applications. In summary,

%\wei{Contributions}
% In summary, our paper delivers a more realistic and comprehensive benchmark for evaluating LLMs' code semantic reasoning capabilities in practical, real-world contexts. We improved the SOTA code benchmarks by 
% \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
% \item defining a spectrum of fine-grained code reasoning tasks that are important for a variety of SE tasks, %i which allows for a more detailed and comprehensive evaluation of a model's capabilities of code semantic reasoning. 
% \item delivering a framework and tool chain that can continuously produce new program traces and detailed code semantics data (mitigating data leakage)  and solved a critical challenge of constructing ground truth for future code reasoning benchmarks design and post-training of the models.
% %fine-grained code semantics ground truth. It is useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.
% \item constructing a benchmark and dataset, consisting of code semantics of real-world software projects of Python, C and Java
% \item investigating six research questions and the SOTA LLMs regarding their capabilities and challenges of code semantic reasoning
% \item placing a leaderboard to make our benchmark immediately available for impacting ongoing LLMs improvement for code tasks. 
% %\item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.
% %\item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
% \end{enumerate}


\wei{I had done a version of intro}



\mycomment{

\TODO{LLM is used for SE applications}
Recently, code large language models (LLMs) have demonstrated great potential in software development tasks such as code generation, testing, and maintenance. These models are trained on massive corpora of both natural and programming languages and are typically evaluated using benchmarks that measure their performance on specific tasks. For instance, HumanEval and DyCodeEval have been proposed to benchmark code generation capabilities. 

\TODO{existing benchmarks do not consider code semantics but understanding code semantics is mandatory for many SE tasks, such as...}
While these existing benchmarks are valuable, they primarily focus on task-specific evaluation rather than assessing a model’s code semantic understanding-—a critical capability for enabling automatic reasoning about program properties. In traditional software development, developers first understand the semantics of the code and then write software accordingly. In contrast, code LLMs often generate code directly, raising an important question: \textit{Do they truly understand the semantics of the code?}
Semantic understanding is especially important for tasks such as test generation and vulnerability detection. As illustrated in \figref{fig:vulnerability-examples}, \TODO{explain the examples}, if code LLMs can accurately comprehend the semantics of the highlighted code snippets, they are more likely to produce correct, secure, and testable code. Enhancing semantic understanding in LLMs could therefore lead to more reliable and effective tools for real-world software engineering.

\TODO{existing work and their limitation}
To explore whether code LLMs are capable of understanding code semantics, a number of code reasoning benchmarks have been proposed. Unlike benchmarks that evaluate real-world task-solving capabilities, these reasoning benchmarks focus on code semantic understanding. For example, \TODO{}. Unfortunately, current code semantics benchmarks have several key limitations that prevent a comprehensive understanding of code LLMs' semantic capabilities:  \textit{1. Non–real-world code sources}: Existing benchmarks are often constructed from synthetic datasets or coding contest problems instead of real-world software repositories. This disconnect limits the benchmarks’ ability to reflect the kinds of semantic patterns and challenges encountered in real-world software engineering. \textit{2. Coarse-grained semantic focus}: Many benchmarks emphasize coarse-grained semantics, typically at the function level. However, coarse granularity fails to capture subtle, fine-grained semantic nuances necessary for reasoning about edge cases. This can be particularly problematic in security-critical scenarios like vulnerability detection, where small semantic misunderstandings can lead to significant failures. \textit{3. Toy semantic tasks}: Existing benchmarks often focus on simplified tasks like input/output prediction or basic code comprehension, which are far removed from the complex reasoning required in real-world SE. As a result, they provide limited insight into a model’s ability to understand and reason about intricate program behaviors.

\TODO{our proposal and highlevel solution} 
To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.

\TODO{implementation and evaluation}

\TODO{contribution}
Our primary contributions are:
\begin{enumerate}

% \item We defined a spectrum of fine-grained code reasoning tasks for evaluating and improving models' understanding of code semantics, which we show are directly linked to handling SE tasks such as test input generation, vulnerability detection, debugging, program repair and code generation. 

% \item We constructed a benchmark and dataset, consisting of real-world software projects in multiple programming languages of C,  python, Java and Javascripts 

% \item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.

% \item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}

\gail{can we say anything at the end of the introduction about a leaderboard?}

\clearpage


\input{Bakeup/intro}
}

==> Bakeup/intro-wei.tex <==
\section{Introduction}
As LLMs significantly improve for software engineering (SE) tasks, we urgently need more advanced and challenging benchmarks for continuously evaluating and improving LLMs. Ideally, a good benchmark should reflect the models' capabilities of solving real-world SE tasks, and the benchmarks are representative such that when models improve over the benchmarks, they should also improve their capabilities of handling other relevant SE tasks. 

%(1) benchmarks like SWE-Bench, Multi-SWE Bench \cite{jimenez2024swebenchlanguagemodelsresolve}, CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning} focus on task-specific evaluation, rather than directly assessing whether a model understands code semantics.  We may learn whether a model performs well for a limited set of end-user tasks such as predicting output given an input, generating patches given a Github issues; but it is unclear if the models achieve high performance on these tasks can be good for other coding tasks, and when models perform poorly, which step prevents the models from achieving better performance. (2) benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}  used synthentic data or educational coding problems, and the evaluation is not centred on real-world software projects. The real-world benchmarks such as SWE-Bench, Multi-SWE Bench face questions whether the models have seen the data.

Currently, we see gaps in code benchmark design: (1) \textit{lacking real-world code sources}:  benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}~\ray{is it also competitive coding benchmark?}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}   used synthetic data or stand-alone competitive coding problems, which do not reflect how developers develop large scale software in real world; %.  and the evaluation is not centered on real-world software projects; 
(2) \textit{focusing on coarse-grained simple reasoning tasks}: benchmarks like 
CruxEval ~\cite{gu2024cruxevalbenchmarkcodereasoning} focused on simple tasks such as input/output prediction at a function level (where functions are simple few lines code using string utility); however, there are many other code reasoning tasks, some of which require to reason about fine-grained, statement level code semantics (3) \textit{evaluating a limited set of end-user tasks}: benchmarks like SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}   
focus on task-specific evaluation rather than directly assessing whether a model understands code semantics. Using such benchmarks, we may learn whether the model performs well for a particular end-user task such as generating patches to resolve a GitHub issue; but it is unclear when the models improve performance on such tasks, whether they can also perform better on many other SE tasks.

%----when models perform poorly, it is hard to understand why and which step that prevents the models from performing better.

%To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.


We propose \bench: (1) it is constructed from real-world GitHub software projects of Python, C and Java, (2) it introduced a spectrum of fine-grained {\it code semantic reasoning tasks} that are essential for a wide range of SE tasks. Using domain knowledge, we identified important, frequently needed code properties across multiple levels of code granularity, statement-level, block-level and function-level. We built a framework and tool chain that can generate ground truth for these fine-grained code reasoning tasks. For example, it is important to reason about loop iterations for input/output prediction, for identifying software performance bottleneck, and for also detecting denial-of-service (infinite loops) attacks. Thus, one of our fine-grained semantic reasoning tasks is to predict the number of loop iterations given an input. As another example, in Figure~\ref{fig:test}, to generate an input to test the dangerous code at line~4, we need the model to understand the code semantics of arithmetic at line~2 and the conditional branch at line~3, so that it can construct a value to set the branch to be {\tt true}. Such statement level code semantic understanding is also important for SE applications like branch prediction and input/output prediction. Similarly, in Figure~\ref{fig:vul}, the models need to understand the semantics of calls {\tt malloc} and {\tt free} at lines~2 and 4, as well as the branch at line 3 o detect whether this code has a memory leak to localize the fault, and to repair it. In the prior literature Traced~\cite{ding2023tracedexecutionawarepretrainingsource} and SemCoder~\cite{ding2024semcodertrainingcodelanguage}, researchers have demonstrated that fine-tuning models with code semantics, the models can improve a variety of SE tasks, including code generation, branch prediction, code clone detection, program repair and vulnerability detection. 

\begin{figure}
% \begin{wrapfigure}{r}{0.65\textwidth}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
void foo(int input){
   int n = input * 23;
  if (n >= 1580){
     //dangerous code need to be tested 
  }
}
    \end{minted}
    \end{tcolorbox}
    \caption{Test input generation and execution reasoning: to generate a test input that can lead to the execution of dangerous code. The model needs to find an input that can make the condition $n\geq$ 1580 true. However, it is hard to generalize across examples, as each program can have different values, without knowing semantics, it is hard to find patterns. Understanding the semantics of operators '*' at line 2 an d'$\geq$' at line 3 is needed to effectively generate test input that reaches dangerous code, e.g., n = 2000 \label{fig:test}}
    \end{subfigure}\quad%
    % 
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3,5,7,8},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
    void bar (int nbits) {
        FFTContext *s = malloc(sizeof (* s));
        if (s && nbits==100))
            free(& s);
         return s;
 }
    \end{minted}
    \end{tcolorbox}
    \caption{Vulnerability detection, fault localization and repair: this code has a memory leak vulnerability when the {\tt if} condition at line~3 is {\tt false}. To detect this vulnerability, it is best that the models know that calls of {\tt malloc} and {\tt free} are related to the vulnerability (semantics of the calls), and should be paired along the program paths along both branches of {\tt if} conditions (semantics of the branch statements). {\tt malloc} and {\tt free} can be located in various code context in different programs, it is hard to generalize the patterns from the code text only without code semantic reasoning.
    \label{fig:vul}}
    \end{subfigure}
    \definecolor{DiffGreen}{HTML}{368B00}
    \definecolor{DiffRed}{HTML}{A51901}
    \caption{Fine-grained code semantics are the keys for precisely solving many SE tasks
    \label{fig:example}}
\end{figure}

%implementation
To construct \bench, we collected 544 Python, 100 C, 110 Java projects, we developed a comprehensive framework to build, execute and collect run-time execution values and traces of the real-world projects. For Python, we executed test cases using the pytest module, and collected execution traces using PySnooper. For C, we used the projects curated in OSS-Fuzz, and the projects were built and fuzzed by OSS-fuzz's docker-based infrastructure. We employed GNU debugger(GDB) to collect run-time traces from C projects. For Java, We used the SF110 dataset, and EvoSuite to generate test cases. We developed the Java tracing framework using the Java Debugger. Using the collected execution trace logs, we build analysis tools to extract the ground truth for our reasoning tasks, and applied filters (details in Section 3) and selected a total of 2125 Python,  1255 C, and 875 Java unique functions in our benchmark.

%we constructed \bench, by extracting the function-level traces and curating benchmark datasets for different code understanding tasks.

%\wei{Roy please add some details regarding our benchmark construction and tools} 

%research question
Using our benchmark, we evaluated  SOTA LLMs and investigated seven research questions regarding models code semantic reasoning capabilities. In the past, we see that models did not perform well on code reasoning tasks such as input/output prediction~\cite{gu2024cruxevalbenchmarkcodereasoning} and vulnerability detection~\cite{steenhoek2025errmachinevulnerabilitydetection}; to understand why models fail and identify places for improvement, we proposed {\bf RQ1}: {\it What types of program statements the model can understand well?  does the model feel any type particularly difficult?}  and {\bf RQ2:} {\it Does increasing the size of code increase the difficulty of code reasoning?}. We identified and evaluated frequently code reasoning tasks shared across many SE tasks, and investigated {\bf RQ3}: {\it How do models perform regarding code properties that are frequently needed for solving SE tasks such as pointer aliasing, loop iterations and values, and branch prediction?} We also studied {\bf RQ4}: {\it How do different prompt techniques help?} and {\bf RQ5}: {\it Any particular programming languages are easier for the models?}. We observed that models face challenges of predicting a precise program value/property, so  we investigated {\bf RQ6}: {\it Can models reason an approximation of code semantics?}. While the code reasoning capabilities of LLMs rapidly improve, to probe we are there yet, we studied {\bf RQ7}: {\it How does the best SOTA LLMs perform our fine-grained code reasoning tasks?}

%results
%\wei{Roy: can you add a summary of results}\\
Our results show that current LLMs lack sufficient knowledge of fine-grained code semantic and as a result, facing challenges to reasoning about even one statement, especially for arithmetic statement and API and function calls, as well as reasoning about important program properties, especially when the answers are not yes/no binary predictions, such as loop values and iterations. The reasoning models, such as, DeepseekR1-distill-Llama-8B, DeepseekR1-distill-Qwen-14B, and the most recent paid models like Claude 3.7, GPT 4o-mini and Gemini-1.5, do not help. and simple COT prompting is not useful. In context-learning prompting helped especially when we selected the in-context shots relevant to our queries, but the improvement is not significant.  We observed that many models feel more difficult when we increased the sizes of code. We observed that across different programming languages, C is the most difficult for output prediction, python is the most for input prediction \wei{Roy, please double check this conclusions}.

%exhibits varying capabilities across different semantic tasks. For RQ1, while the models show higher prediction accuracy for statements like Constant Assignment and branch statements, they struggle with tasks which involve function calls and arithmetic. We also observed that increasing block sizes resulted in a decrease in performance for the models (RQ2). 


%Our goal of designing \bench is to improve the state-of-the-art (SOTA) code benchmarks by (1) defining a spectrum of code semantic reasoning tasks that are important for a variety of SE tasks (2) delivering a framework and tool chain that can continuously produce new program traces and construct ground truth for code semantics for real-world software projects consisting of Python, C and Java, useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.


%his paper presents a comprehensive study and real-world multi-lingual benchmark, dataset and framework tools that can evaluate the future models. It's the first this paper is first that defines the code reasoning capabilities via a spectum of fine-grained code reasoning tasks that directly link to important SE applications. In summary,

%\wei{Contributions}
In summary, our paper delivers a more realistic and comprehensive benchmark for evaluating LLMs' code semantic reasoning capabilities in practical, real-world contexts. We improved the SOTA code benchmarks by 
\begin{enumerate}
\item defining a spectrum of fine-grained code reasoning tasks that are important for a variety of SE tasks, %i which allows for a more detailed and comprehensive evaluation of a model's capabilities of code semantic reasoning. 
\item delivering a framework and tool chain that can continuously produce new program traces and detailed code semantics data (thus avoiding data leakage)  and solved a critical challenge of constructing ground truth for future code reasoning benchmarks design and post-training of the models.
%fine-grained code semantics ground truth. It is useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.
\item constructing a benchmark and dataset, consisting of code semantics of real-world software projects of Python, C and Java
\item investigating seven research questions and the SOTA LLMs regarding their capabilities and challenges of code semantic reasoning
\item placing a leaderboard to make our benchmark immediately available for impacting ongoing LLMs improvement for code tasks. 
%\item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.
%\item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}


\wei{I had done a version of intro}



\mycomment{

\TODO{LLM is used for SE applications}
Recently, code large language models (LLMs) have demonstrated great potential in software development tasks such as code generation, testing, and maintenance. These models are trained on massive corpora of both natural and programming languages and are typically evaluated using benchmarks that measure their performance on specific tasks. For instance, HumanEval and DyCodeEval have been proposed to benchmark code generation capabilities. 

\TODO{existing benchmarks do not consider code semantics but understanding code semantics is mandatory for many SE tasks, such as...}
While these existing benchmarks are valuable, they primarily focus on task-specific evaluation rather than assessing a model’s code semantic understanding-—a critical capability for enabling automatic reasoning about program properties. In traditional software development, developers first understand the semantics of the code and then write software accordingly. In contrast, code LLMs often generate code directly, raising an important question: \textit{Do they truly understand the semantics of the code?}
Semantic understanding is especially important for tasks such as test generation and vulnerability detection. As illustrated in \figref{fig:vulnerability-examples}, \TODO{explain the examples}, if code LLMs can accurately comprehend the semantics of the highlighted code snippets, they are more likely to produce correct, secure, and testable code. Enhancing semantic understanding in LLMs could therefore lead to more reliable and effective tools for real-world software engineering.

\TODO{existing work and their limitation}
To explore whether code LLMs are capable of understanding code semantics, a number of code reasoning benchmarks have been proposed. Unlike benchmarks that evaluate real-world task-solving capabilities, these reasoning benchmarks focus on code semantic understanding. For example, \TODO{}. Unfortunately, current code semantics benchmarks have several key limitations that prevent a comprehensive understanding of code LLMs' semantic capabilities:  \textit{1. Non–real-world code sources}: Existing benchmarks are often constructed from synthetic datasets or coding contest problems instead of real-world software repositories. This disconnect limits the benchmarks’ ability to reflect the kinds of semantic patterns and challenges encountered in real-world software engineering. \textit{2. Coarse-grained semantic focus}: Many benchmarks emphasize coarse-grained semantics, typically at the function level. However, coarse granularity fails to capture subtle, fine-grained semantic nuances necessary for reasoning about edge cases. This can be particularly problematic in security-critical scenarios like vulnerability detection, where small semantic misunderstandings can lead to significant failures. \textit{3. Toy semantic tasks}: Existing benchmarks often focus on simplified tasks like input/output prediction or basic code comprehension, which are far removed from the complex reasoning required in real-world SE. As a result, they provide limited insight into a model’s ability to understand and reason about intricate program behaviors.

\TODO{our proposal and highlevel solution} 
To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.

\TODO{implementation and evaluation}

\TODO{contribution}
Our primary contributions are:
\begin{enumerate}

% \item We defined a spectrum of fine-grained code reasoning tasks for evaluating and improving models' understanding of code semantics, which we show are directly linked to handling SE tasks such as test input generation, vulnerability detection, debugging, program repair and code generation. 

% \item We constructed a benchmark and dataset, consisting of real-world software projects in multiple programming languages of C,  python, Java and Javascripts 

% \item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.

% \item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}

\gail{can we say anything at the end of the introduction about a leaderboard?}

\clearpage


\input{Bakeup/intro}
}

==> Bakeup/intro.bck.tex <==
\section{Introduction}
As LLMs significantly improve for software engineering (SE) tasks, we urgently need more advanced and challenging benchmarks for continuously evaluating and improving LLMs. Ideally, a good benchmark should reflect the models' capabilities of solving real-world SE tasks, and the benchmarks are representative such that when models improve over the benchmarks, they should also improve the capabilities of handling other relevant SE tasks. 

%(1) benchmarks like SWE-Bench, Multi-SWE Bench \cite{jimenez2024swebenchlanguagemodelsresolve}, CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning} focus on task-specific evaluation, rather than directly assessing whether a model understands code semantics.  We may learn whether a model performs well for a limited set of end-user tasks such as predicting output given an input, generating patches given a Github issues; but it is unclear if the models achieve high performance on these tasks can be good for other coding tasks, and when models perform poorly, which step prevents the models from achieving better performance. (2) benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}  used synthentic data or educational coding problems, and the evaluation is not centred on real-world software projects. The real-world benchmarks such as SWE-Bench, Multi-SWE Bench face questions whether the models have seen the data.

Currently, we see gaps in code benchmark design: (1) \textit{lacking real-world code sources}:  benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}~\ray{is it also competitive coding benchmark?}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}   used synthetic data or stand-alone competitive coding problems, which do not reflect how developers develop large scale software in real world; %.  and the evaluation is not centered on real-world software projects; 
(2) \textit{focusing on coarse-grained simple reasoning tasks}: benchmarks like 
CruxEval ~\cite{gu2024cruxevalbenchmarkcodereasoning} focused on simple tasks such as input/output prediction at a function level (where functions are simple few lines code using string utility); however, there are many other code reasoning tasks, many of which require to reason about fine-grained code semantics like the values of statements and properties within a function (3) \textit{for real-world code, only evaluating very few end-user tasks}: benchmarks like SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}   
focus on task-specific evaluation rather than directly assessing whether a model understands code semantics. Using such benchmarks, we may learn whether the model performs well for a particular end-user task such as generating patches to resolve a GitHub issue; but it is unclear when the models improve performance on such tasks, whether they can also perform better on many other SE tasks.

%----when models perform poorly, it is hard to understand why and which step that prevents the models from performing better.

%To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.


We propose \bench: (1) it is constructed from real-world GitHub software projects of Python, C/C++ and Java, (2) it introduced a spectrum of fine-grained {\it code semantic reasoning tasks} that are essential for a wide range of SE tasks. Using domain knowledge, we identified important, frequently needed code properties across multiple levels of code granularity, statement-level, block-level and function-level. We built a framework and tool chain that can generate ground truth for such fine-grained code reasoning tasks. For example, it is important to reason about loop iterations for input/output prediction, for identifying software performance bottleneck, and for also detecting denial-of-service (infinite loops) attacks. Thus, one of our fine-grained semantic reasoning tasks is to predict the number of loop iterations given an input. As another example, in Figure~\ref{fig:test}, to generate an input to test the dangerous code at line~4, we need the model to understand the code semantics of arithmetic at line~2 and the conditional branch at line~3, so that it can construct a value to set the branch to be {\tt true}. Such statement level code semantic understanding is also important for SE applications like branch prediction and input/output prediction. Similarly, in Figure~\ref{fig:vul}, the models need to understand the semantics of calls {\tt malloc} and {\tt free} at lines~2 and 4, as well as the branch at line 3 o detect whether this code has a memory leak to localize the fault, and to repair it. In the prior literature Traced~\cite{ding2023tracedexecutionawarepretrainingsource} and SemCoder~\cite{ding2024semcodertrainingcodelanguage}, researchers have demonstrated that fine-tuning models with code semantics, the models can improve a variety of SE tasks, including code generation, branch prediction, code clone detection, program repair and vulnerability detection. 

\begin{figure}
% \begin{wrapfigure}{r}{0.65\textwidth}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
void foo(int input){
   int n = input * 23;
  if (n >= 1580){
     //dangerous code need to be tested 
  }
}
    \end{minted}
    \end{tcolorbox}
    \caption{Test input generation and execution reasoning: to generate a test input that can lead to the execution of dangerous code. The model needs to find an input that can make the condition $n\geq$ 1580 true. However, it is hard to generalize across examples, as each program can have different values, without knowing semantics, it is hard to find patterns. Understanding the semantics of 'x' at line 2 an d'$\geq$' at line 3 is needed to effectively generate test input that reaches dangerous code, e.g., n = 2000 \label{fig:test}}
    \end{subfigure}\quad%
    % 
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3,5,7,8},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
    void bar (int nbits) {
        FFTContext *s = malloc(sizeof (* s));
        if (s && nbits==100))
            free(& s);
         return s;
 }
    \end{minted}
    \end{tcolorbox}
    \caption{Vulnerability detection, fault localization and repair: This code has a memory leak vulnerability when the if condition at line~4 is false. To detect this vulnerability, models need to know malloc and free should be paired along the program paths, but here when if is false at line~4, the memory leak can happen. It is hard to generalize the patterns beause there can be many ifs before free.
    \label{fig:vul}}
    \end{subfigure}
    \definecolor{DiffGreen}{HTML}{368B00}
    \definecolor{DiffRed}{HTML}{A51901}
    \caption{Examples of vulnerability detection as a complex code reasoning task. Diffed lines (\textbf{{\color{DiffGreen}+}}/\textbf{{\color{DiffRed}-}}) show the lines changed to patch the vulnerability.

    \label{fig:vulnerability-examples}}
\end{figure}

%implementation
To construct \bench, we collected 544 Python, 100 C/C++, 110 Java projects, we developed a comprehensive framework to build, execute and collect run-time execution values and traces of the real-world projects. For Python, we executed test cases using the pytest module, and collected execution traces using PySnooper. For C, we used the projects curated in OSS-Fuzz, and the projects were built and fuzzed by OSS-fuzz's docker-based infrastructure. We employed GNU debugger(GDB) to collect run-time traces from C projects. For Java, We used the SF110 dataset, and EvoSuite to generate test cases. We developed the Java tracing framework using the Java Debugger. Using the collected statement-level execution trace logs, we extracted the ground truth and selected a total of programs as benchmarks. 

%we constructed \bench, by extracting the function-level traces and curating benchmark datasets for different code understanding tasks.

\wei{Roy please add some details regarding our benchmark construction and tools} 

%research question
Using our benchmark, we evaluated  SOTA LLMs and investigated seven research questions. In the past, we see that models did not perform well on code reasoning tasks such as input/output prediction~\cite{gu2024cruxevalbenchmarkcodereasoning} and vulnerability detection~\cite{ben}, to understand why models fail and what are the challenges of the models, we proposed fine-grain investigations on 
{\bf RQ1}: What types of program statements the model can understand well?  does the model feel any type particularly difficult?  and {\bf RQ2:} Does increasing the size of code increase the difficulty of code reasoning? We highlighted and evaluated frequently code reasoning steps that are important for many SE tasks. {\bf RQ3}: How do model perform regarding queries that are frequently needed for solving SE tasks such as properties related to loops and pointers? Besides zero-shot, the easist and common application scenarios we investigated {\bf RQ4}: How do different prompt techniques perform? and {\bf RQ5}: Any particular programming languages are easier for the models? Considering predicting a precise value can be challenging, we also investigated whether we can {\bf RQ6}: Can models handle approximation of code semantics? and {\bf RQ7}: How does the best SOTA LLMs perform the tasks. 

%results
\wei{Roy: can you add a summary of results} Our results show that 


%Our goal of designing \bench is to improve the state-of-the-art (SOTA) code benchmarks by (1) defining a spectrum of code semantic reasoning tasks that are important for a variety of SE tasks (2) delivering a framework and tool chain that can continuously produce new program traces and construct ground truth for code semantics for real-world software projects consisting of Python, C and Java, useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.


%his paper presents a comprehensive study and real-world multi-lingual benchmark, dataset and framework tools that can evaluate the future models. It's the first this paper is first that defines the code reasoning capabilities via a spectum of fine-grained code reasoning tasks that directly link to important SE applications. In summary,

%\wei{Contributions}
In summary, this paper delivers a more realistic and comprehensive benchmark for evaluating LLMs' code semantic reasoning capabilities in practical, real-world contexts. We improved the SOTA code benchmarks by 
\begin{enumerate}
\item defining a spectrum of fine-grained code reasoning tasks  that are important for a variety of SE tasks  which allows for a more detailed and comprehensive evaluation of a model's capabilities of code semantic reasoning. 
\item delivering a framework and tool chain that can continuously produce new program traces and construct ground truth for code semantics for real-world software projects consisting of Python, C and Java. This tool chain solved an important challenge of constructing fine-grained code semantics ground truth. It is useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.
\item constructing a benchmark and dataset, consisting of real-world software projects in multiple programming languages of C,  python, Java and Javascripts 
\item investigating seven reason questions and the SOTA LLMs regarding their capabilities and challenges of code semantic reasoning
\item placing a leader board for directly impacting the ongoing LLMs improvement for code tasks. 
\item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.
\item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\item We have prepared a leaderboard 
\end{enumerate}


\wei{drafting a version of intro}





\TODO{LLM is used for SE applications}
Recently, code large language models (LLMs) have demonstrated great potential in software development tasks such as code generation, testing, and maintenance. These models are trained on massive corpora of both natural and programming languages and are typically evaluated using benchmarks that measure their performance on specific tasks. For instance, HumanEval and DyCodeEval have been proposed to benchmark code generation capabilities. 

\TODO{existing benchmarks do not consider code semantics but understanding code semantics is mandatory for many SE tasks, such as...}
While these existing benchmarks are valuable, they primarily focus on task-specific evaluation rather than assessing a model’s code semantic understanding-—a critical capability for enabling automatic reasoning about program properties. In traditional software development, developers first understand the semantics of the code and then write software accordingly. In contrast, code LLMs often generate code directly, raising an important question: \textit{Do they truly understand the semantics of the code?}
Semantic understanding is especially important for tasks such as test generation and vulnerability detection. As illustrated in \figref{fig:vulnerability-examples}, \TODO{explain the examples}, if code LLMs can accurately comprehend the semantics of the highlighted code snippets, they are more likely to produce correct, secure, and testable code. Enhancing semantic understanding in LLMs could therefore lead to more reliable and effective tools for real-world software engineering.

\TODO{existing work and their limitation}
To explore whether code LLMs are capable of understanding code semantics, a number of code reasoning benchmarks have been proposed. Unlike benchmarks that evaluate real-world task-solving capabilities, these reasoning benchmarks focus on code semantic understanding. For example, \TODO{}. Unfortunately, current code semantics benchmarks have several key limitations that prevent a comprehensive understanding of code LLMs' semantic capabilities:  \textit{1. Non–real-world code sources}: Existing benchmarks are often constructed from synthetic datasets or coding contest problems instead of real-world software repositories. This disconnect limits the benchmarks’ ability to reflect the kinds of semantic patterns and challenges encountered in real-world software engineering. \textit{2. Coarse-grained semantic focus}: Many benchmarks emphasize coarse-grained semantics, typically at the function level. However, coarse granularity fails to capture subtle, fine-grained semantic nuances necessary for reasoning about edge cases. This can be particularly problematic in security-critical scenarios like vulnerability detection, where small semantic misunderstandings can lead to significant failures. \textit{3. Toy semantic tasks}: Existing benchmarks often focus on simplified tasks like input/output prediction or basic code comprehension, which are far removed from the complex reasoning required in real-world SE. As a result, they provide limited insight into a model’s ability to understand and reason about intricate program behaviors.

\TODO{our proposal and highlevel solution} 
To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.

\TODO{implementation and evaluation}

\TODO{contribution}
Our primary contributions are:
\begin{enumerate}

% \item We defined a spectrum of fine-grained code reasoning tasks for evaluating and improving models' understanding of code semantics, which we show are directly linked to handling SE tasks such as test input generation, vulnerability detection, debugging, program repair and code generation. 

% \item We constructed a benchmark and dataset, consisting of real-world software projects in multiple programming languages of C,  python, Java and Javascripts 

% \item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.

% \item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}

\gail{can we say anything at the end of the introduction about a leaderboard?}

\clearpage

\input{Bakeup/intro}

==> Bakeup/results-Wei.tex <==
\wei{Future work: Good to add findings and interesting examples to RQs}
\wei{future work: it will be interesting to do individual statement input prediction}
\wei{future work:  supporting more datatypes arrays, matrix, strings }

\wei{future work: it is interesting to experiment when block 2 is wrong, how the individual statement prediction in the block performs? Is it because the model can't predict statements in the block or it cannot predict the progression/connection of the two statements}

==> Text/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The summarization of the paper's contribution and novelty is in Abstract and Introduction (Section~\ref{sec:intro})
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include them in the appendix \ref{app:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no theoretical results in this work since our results focus on constructing code semantics benchmark for LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have explained the configuration of our implementation and configuration in appendix \ref{app:computation}. We will also release the reproducible artifact publicly.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our data, code, and models are available at: \url{https://codesense-bench.github.io/}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: We include data collection and experimental configuration in Section~\ref{Benchmark} and Section~\ref{Evaluation} and in appendix ~\ref{app:computation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed them in Section~\ref{Benchmark} and Section~\ref{Evaluation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provided the information in appendix \ref{app:computation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We checked the code of ethics and ensure our research algins with the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: There is no potential positive or negative societal impacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification:  The paper does not release any data, models, or resources that could be considered high-risk for misuse. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have properly cited all the tools, data and models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our documents will be available at \url{https://codesense-bench.github.io/}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: There's no crowdsourcing nor human subjects in our paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: There's no crowdsourcing nor human subjects in our paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> Text/checklist_dataset.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have extensively used \sys and \data proposed in the paper to conduct more than $30$k kernel experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper states that we perform only baseline experiments on kernel crash resolution and admits that there exists much scope for additional research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no theoretical results mentioned in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:\answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{subsection:kernel_arch} details the entire process of running \sys's end-to-end pipeline. For each bug in \data, we provide in a JSON file all the necessary metadata to run the kernel experiment - such as the \texttt{Reproducer}, \texttt{Config}, \texttt{Commit\textsubscript{parent}} and \texttt{Crash\textsubscript{parent}}.
    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We plan to open-source the code for \sys and openly release the \data dataset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In our experiments, we only use a test set and do not perform any pre-training or fine-tuning as \data is a low-resource dataset. We have provided a thorough analysis of the test set in Section \ref{sec:kbench_info}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not report error bars in our prompting experiments due to budget constraints. As the prompt for each bug in \data runs into tens of thousands of tokens, repetitively querying state-of-the-art LLMs is prohibitively expensive. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We mention the number (and type) of VMs used when running \sys for all the kernel experiments. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have followed all ethical guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no societal impact of \sys and \data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The data used in \data is directly scraped from the Syzkaller website. In the provided data dump, we only include specific HTML links to certain files hosted on the Syzkaller website and a script that uses these links to download all these files. Hence we do not violate any license terms. In our codebase, we also use and modify repositories having the MIT License. We have made sure to respect the terms of this License. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We open-source \sys under the MIT License and provide detailed documentation along with it. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> Text/intro.bck.tex <==
\section{Introduction}
As LLMs significantly improve for software engineering (SE) tasks, we urgently need more advanced and challenging benchmarks for continuously evaluating and improving LLMs. Ideally, a good benchmark should reflect the models' capabilities of solving real-world SE tasks, and the benchmarks are representative such that when models improve over the benchmarks, they should also improve their capabilities of handling other relevant SE tasks. 

%(1) benchmarks like SWE-Bench, Multi-SWE Bench \cite{jimenez2024swebenchlanguagemodelsresolve}, CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning} focus on task-specific evaluation, rather than directly assessing whether a model understands code semantics.  We may learn whether a model performs well for a limited set of end-user tasks such as predicting output given an input, generating patches given a Github issues; but it is unclear if the models achieve high performance on these tasks can be good for other coding tasks, and when models perform poorly, which step prevents the models from achieving better performance. (2) benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}  used synthentic data or educational coding problems, and the evaluation is not centred on real-world software projects. The real-world benchmarks such as SWE-Bench, Multi-SWE Bench face questions whether the models have seen the data.

Currently, we see gaps in code benchmark design: (1) \textit{lacking real-world code sources}:  benchmarks like CruxEval \cite{gu2024cruxevalbenchmarkcodereasoning}, HumanEval+ \cite{liu2023codegeneratedchatgptreally}, LiveCodeBenchmark \cite{jain2024livecodebenchholisticcontaminationfree}, Bigcodebench \cite{zhuo2024bigcodebenchbenchmarkingcodegeneration}~\ray{is it also competitive coding benchmark?}, CodeBenchGen \cite{xie2024codebenchgencreatingscalableexecutionbased}   used synthetic data or stand-alone competitive coding problems, which do not reflect how developers develop large scale software in real world; %.  and the evaluation is not centered on real-world software projects; 
(2) \textit{focusing on coarse-grained simple reasoning tasks}: benchmarks like 
CruxEval ~\cite{gu2024cruxevalbenchmarkcodereasoning} focused on simple tasks such as input/output prediction at a function level (where functions are simple few lines code using string utility);  however, there are many other code reasoning tasks, many of which require to reason about fine-grained code semantics like the values of statements and properties within a function (3) \textit{evaluating a limited set of end-user tasks for real-world code}:  SWE-Bench ~\cite{jimenez2024swebenchlanguagemodelsresolve}, Swe-PolyBench ~\cite{rashid2025swepolybenchmultilanguagebenchmarkrepository}, and KGym~\cite{mathai2024kgym}  are the benchmarks we found that use real-world code (to the best of our knowledge). However, these benchmarks focus on task-specific evaluation rather than directly assessing whether a model understands code semantics. Using such benchmarks, we may learn whether the model performs well for a particular end-user task such as generating patches to resolve a GitHub issue; but it is unclear when the models improve performance on such tasks, whether they can also perform better on many other SE tasks.

%----when models perform poorly, it is hard to understand why and which step that prevents the models from performing better.

%To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.


We propose \bench: (1) it is constructed from real-world GitHub software projects of Python, C and Java, (2) it introduced a spectrum of fine-grained {\it code semantic reasoning tasks} that are essential for a wide range of SE tasks. Using domain knowledge, we identified important, frequently needed code properties across multiple levels of code granularity, statement-level, block-level and function-level. We built a framework and tool chain that can generate ground truth for these fine-grained code reasoning tasks. For example, it is important to reason about loop iterations for input/output prediction, for identifying software performance bottleneck, and for also detecting denial-of-service (infinite loops) attacks. Thus, one of our fine-grained semantic reasoning tasks is to predict the number of loop iterations given an input. As another example, in Figure~\ref{fig:test}, to generate an input to test the dangerous code at line~4, we need the model to understand the code semantics of arithmetic at line~2 and the conditional branch at line~3, so that it can construct a value to set the branch to be {\tt true}. Such statement level code semantic understanding is also important for SE applications like branch prediction and input/output prediction. Similarly, in Figure~\ref{fig:vul}, the models need to understand the semantics of calls {\tt malloc} and {\tt free} at lines~2 and 4, as well as the branch at line 3 o detect whether this code has a memory leak to localize the fault, and to repair it. In the prior literature Traced~\cite{ding2023tracedexecutionawarepretrainingsource} and SemCoder~\cite{ding2024semcodertrainingcodelanguage}, researchers have demonstrated that fine-tuning models with code semantics, the models can improve a variety of SE tasks, including code generation, branch prediction, code clone detection, program repair and vulnerability detection. 

\begin{figure}
% \begin{wrapfigure}{r}{0.65\textwidth}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
void foo(int input){
   int n = input * 23;
  if (n >= 1580){
     //dangerous code need to be tested 
  }
}
    \end{minted}
    \end{tcolorbox}
    \caption{Test input generation and execution reasoning: to generate a test input that can lead to the execution of dangerous code. The model needs to find an input that can make the condition $n\geq$ 1580 true. However, it is hard to generalize across examples, as each program can have different values, without knowing semantics, it is hard to find patterns. Understanding the semantics of operators '*' at line 2 an d'$\geq$' at line 3 is needed to effectively generate test input that reaches dangerous code, e.g., n = 2000 \label{fig:test}}
    \end{subfigure}\quad%
    % 
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \begin{tcolorbox}
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\tiny,
    highlightlines={3,5,7,8},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    breaklines,
    ]
    {diff}
    void bar (int nbits) {
        FFTContext *s = malloc(sizeof (* s));
        if (s && nbits==100))
            free(& s);
         return s;
 }
    \end{minted}
    \end{tcolorbox}
    \caption{Vulnerability detection, fault localization and repair: this code has a memory leak vulnerability when the {\tt if} condition at line~3 is {\tt false}. To detect this vulnerability, it is best that the models know that calls of {\tt malloc} and {\tt free} are related to the vulnerability (semantics of the calls), and should be paired along the program paths along both branches of {\tt if} conditions (semantics of the branch statements). {\tt malloc} and {\tt free} can be located in various code context in different programs, it is hard to generalize the patterns from the code text only without code semantic reasoning.
    \label{fig:vul}}
    \end{subfigure}
    \definecolor{DiffGreen}{HTML}{368B00}
    \definecolor{DiffRed}{HTML}{A51901}
    \caption{Fine-grained code semantics are the keys for solving many SE tasks
    \label{fig:example}}
\end{figure}

%implementation
To construct \bench, we collected 544 Python, 100 C, 110 Java projects, we developed a comprehensive framework to build, execute and collect run-time execution values and traces of the real-world projects. For Python, we executed test cases using the pytest module, and collected execution traces using PySnooper. For C, we used the projects curated in OSS-Fuzz, and the projects were built and fuzzed by OSS-fuzz's docker-based infrastructure. We employed GNU debugger(GDB) to collect run-time traces from C projects. For Java, We used the SF110 dataset, and EvoSuite to generate test cases. We developed the Java tracing framework using the Java Debugger. Using the collected execution trace logs, we build analysis tools to extract the ground truth for our reasoning tasks, and applied filters (details in Section 3) and selected a total of 2125 Python,  1255 C, and 875 Java unique functions in our benchmark.

%we constructed \bench, by extracting the function-level traces and curating benchmark datasets for different code understanding tasks.

%\wei{Roy please add some details regarding our benchmark construction and tools} 

%research question
Using our benchmark, we evaluated  SOTA LLMs and investigated six research questions regarding models code semantic reasoning capabilities. In the past, we see that models did not perform well on code reasoning tasks such as input/output prediction~\cite{gu2024cruxevalbenchmarkcodereasoning} and vulnerability detection~\cite{steenhoek2025errmachinevulnerabilitydetection}; to understand why models fail and identify places for improvement, we proposed {\bf RQ1}: {\it What types of program statements the model can understand well?  does the model feel any type particularly difficult?}  and {\bf RQ2:} {\it Does increasing the size of code increase the difficulty of code reasoning?}. We identified and evaluated frequently code reasoning tasks shared across many SE tasks, and investigated {\bf RQ3}: {\it How do models perform regarding code properties that are frequently needed for solving SE tasks such as pointer aliasing, loop iterations and values, and branch prediction?} We also studied {\bf RQ4}: {\it How do different prompt techniques help?} and {\bf RQ5}: {\it Any particular programming languages are easier for the models?}. We observed that models face challenges of predicting a precise program value/property, so  we investigated {\bf RQ6}: {\it Can models reason about an approximation of code semantics?}. %While the code reasoning capabilities of LLMs rapidly improve, to probe we are there yet, we studied {\bf RQ7}: {\it How does the best SOTA LLMs perform our fine-grained code reasoning tasks?}

%results
%\wei{Roy: can you add a summary of results}\\
Our results show that current LLMs lack sufficient knowledge of fine-grained code semantics and face challenges of reasoning for even one statement from real-world code, especially for arithmetic statements and API/calls. LLMs also generally reported low performance for reasoning about program properties such as loop values and iterations. The reasoning models and the state-of-the-art big models like Claude 3.7, GPT 4o-mini and Gemini-1.5, do not help much.  Simple COT prompting is not useful. 


Interestingly, the models do know some semantics for the frequently occurred code patterns, like when the code text contains an assignment "p=q", and our prompt explained that "two aliased pointers have the same memory addresses", the models are able to return {\tt p} and {\tt q} are aliased even in the zero-shot setting. Similarly, when our prompt asked the model to answer the number of loop iterations, the models often know they should report 100 if the code contains the loop {\tt for i in range(100):}. In context-learning prompting helped especially when we selected the in-context shots relevant to our queries, but the improvement is not significant. It is especially useful when we introduce a newly defined concept in the prompt, e.g., when we asked models to predict "abstract values" and we define what we mean by abstract values in the prompt. Among the 14 SOTA models we studied, we found that Claude 3.7 overall performed best in our fine-grained reasoning tasks.  We found that compared to C code, Java/Python are easier for models to predict output given input. Models have very little knowledge on "reverse" code semantcs, and input predictions becomes the most difficult tasks.

\mycomment{
We observed that reasoning is more difficult when the code size increase. We observed that across different programming languages, C is the most difficult for output prediction, python is the most for input prediction \wei{Roy, please double check this conclusions}. 
Good models: Claude, better models for all tasks  Granaite models
\wei{will  Models are able to link natural language in our prompt with code patterns, e.g., }
}

%exhibits varying capabilities across different semantic tasks. For RQ1, while the models show higher prediction accuracy for statements like Constant Assignment and branch statements, they struggle with tasks which involve function calls and arithmetic. We also observed that increasing block sizes resulted in a decrease in performance for the models (RQ2). 


%Our goal of designing \bench is to improve the state-of-the-art (SOTA) code benchmarks by (1) defining a spectrum of code semantic reasoning tasks that are important for a variety of SE tasks (2) delivering a framework and tool chain that can continuously produce new program traces and construct ground truth for code semantics for real-world software projects consisting of Python, C and Java, useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.


%his paper presents a comprehensive study and real-world multi-lingual benchmark, dataset and framework tools that can evaluate the future models. It's the first this paper is first that defines the code reasoning capabilities via a spectum of fine-grained code reasoning tasks that directly link to important SE applications. In summary,

%\wei{Contributions}
In summary, our paper delivers a more realistic and comprehensive benchmark for evaluating LLMs' code semantic reasoning capabilities in practical, real-world contexts. We improved the SOTA code benchmarks by 
\begin{enumerate}
\item defining a spectrum of fine-grained code reasoning tasks that are important for a variety of SE tasks, %i which allows for a more detailed and comprehensive evaluation of a model's capabilities of code semantic reasoning. 
\item delivering a framework and tool chain that can continuously produce new program traces and detailed code semantics data (mitigating data leakage)  and solved a critical challenge of constructing ground truth for future code reasoning benchmarks design and post-training of the models.
%fine-grained code semantics ground truth. It is useful for designing future benchmarks and fine-tune models. Using such newly generated data for evaluation, the models will not face the data-leakage problems that benchmarks commonly face.
\item constructing a benchmark and dataset, consisting of code semantics of real-world software projects of Python, C and Java
\item investigating six research questions and the SOTA LLMs regarding their capabilities and challenges of code semantic reasoning
\item placing a leaderboard to make our benchmark immediately available for impacting ongoing LLMs improvement for code tasks. 
%\item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.
%\item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}


\wei{I had done a version of intro}



\mycomment{

\TODO{LLM is used for SE applications}
Recently, code large language models (LLMs) have demonstrated great potential in software development tasks such as code generation, testing, and maintenance. These models are trained on massive corpora of both natural and programming languages and are typically evaluated using benchmarks that measure their performance on specific tasks. For instance, HumanEval and DyCodeEval have been proposed to benchmark code generation capabilities. 

\TODO{existing benchmarks do not consider code semantics but understanding code semantics is mandatory for many SE tasks, such as...}
While these existing benchmarks are valuable, they primarily focus on task-specific evaluation rather than assessing a model’s code semantic understanding-—a critical capability for enabling automatic reasoning about program properties. In traditional software development, developers first understand the semantics of the code and then write software accordingly. In contrast, code LLMs often generate code directly, raising an important question: \textit{Do they truly understand the semantics of the code?}
Semantic understanding is especially important for tasks such as test generation and vulnerability detection. As illustrated in \figref{fig:vulnerability-examples}, \TODO{explain the examples}, if code LLMs can accurately comprehend the semantics of the highlighted code snippets, they are more likely to produce correct, secure, and testable code. Enhancing semantic understanding in LLMs could therefore lead to more reliable and effective tools for real-world software engineering.

\TODO{existing work and their limitation}
To explore whether code LLMs are capable of understanding code semantics, a number of code reasoning benchmarks have been proposed. Unlike benchmarks that evaluate real-world task-solving capabilities, these reasoning benchmarks focus on code semantic understanding. For example, \TODO{}. Unfortunately, current code semantics benchmarks have several key limitations that prevent a comprehensive understanding of code LLMs' semantic capabilities:  \textit{1. Non–real-world code sources}: Existing benchmarks are often constructed from synthetic datasets or coding contest problems instead of real-world software repositories. This disconnect limits the benchmarks’ ability to reflect the kinds of semantic patterns and challenges encountered in real-world software engineering. \textit{2. Coarse-grained semantic focus}: Many benchmarks emphasize coarse-grained semantics, typically at the function level. However, coarse granularity fails to capture subtle, fine-grained semantic nuances necessary for reasoning about edge cases. This can be particularly problematic in security-critical scenarios like vulnerability detection, where small semantic misunderstandings can lead to significant failures. \textit{3. Toy semantic tasks}: Existing benchmarks often focus on simplified tasks like input/output prediction or basic code comprehension, which are far removed from the complex reasoning required in real-world SE. As a result, they provide limited insight into a model’s ability to understand and reason about intricate program behaviors.

\TODO{our proposal and highlevel solution} 
To address the limitations of existing work and enable fine-grained semantic understanding in real-world software projects, we propose \tool. Unlike prior benchmarks based on synthetic or educational data, \tool collects its codebase directly from real-world GitHub projects, thereby addressing the first limitation related to unrealistic data sources. To overcome the second limitation—-coarse-grained semantic evaluation—-\tool introduces a diverse set of semantic understanding tasks across multiple levels of granularity, addressing statement-level, block-level, and function-level reasoning. This allows for a more detailed and layered evaluation of a model's semantic capabilities. In addition, \tool incorporates two critical code property reasoning tasks: loop analysis and pointer analysis. These tasks are essential and widely applicable in real-world SE. For example, loop analysis can be used to reason about software performance, while pointer analysis plays a key role in detecting memory safety issues and vulnerabilities. Together, these design choices allow \tool to provide a more realistic and comprehensive benchmark for evaluating the semantic understanding of code LLMs in practical, real-world contexts.

\TODO{implementation and evaluation}

\TODO{contribution}
Our primary contributions are:
\begin{enumerate}

% \item We defined a spectrum of fine-grained code reasoning tasks for evaluating and improving models' understanding of code semantics, which we show are directly linked to handling SE tasks such as test input generation, vulnerability detection, debugging, program repair and code generation. 

% \item We constructed a benchmark and dataset, consisting of real-world software projects in multiple programming languages of C,  python, Java and Javascripts 

% \item We developed frameworks and tools that enable automatic collection of fine-grained code execution data for future generation of data and bechnmarks. The data including program input/output, intermediate values, traces and program properties like loop counters. This framework can be used to generate further program execution data an benchmarks.

% \item We performed systematic evaluate on the models' capabilities of understanding code semantics and present interesting findings.
\end{enumerate}

\gail{can we say anything at the end of the introduction about a leaderboard?}

\clearpage


\input{Bakeup/intro}
}
